Atomic Higgsings of 6D SCFTs II: Induced Flows

We study a specific type of atomic Higgsings of the 6d $\mathcal{N}=(1,0)$ theories, which we call the induced flows. For the conformal matter theory associated with a pair of nilpotent orbits, the induced flows are given by the inductions of the orbits. We also consider the induced flows for the orbi-instanton theories (as well as some little string theories) that are associated with the homomorphisms from the discrete subgroups of $\mathrm{SU}(2)$ to $E_8$. This gives a physical definition of the inductions among these discrete homomorphisms, analogous to the inductions of the nilpotent orbits. We analyze the Higgs branch dimensions, the monotonicity of the Weyl anomalies (or the 2-group structure constants for LSTs) and the brane pictures under the induced flows.

==> response2.tex <==
We would like to thank the referee for the further comments that would help us clarify the discussions in the paper. Here are the changes we have made:

3. We added the explanation in footnote 4 on page 4. The T-brane data should be identified as the period of certain 3-form potential for the Calabi-Yau threefold as identified in Ref.~[34].

8. We added a figure for the Type IIA picture in Figure 2.3 to illustrate that the Higgsing is not atomic.

We hope that these changes could implement the comments by the referee.
